QAdaPrune: Adaptive Parameter Pruning For Training Variational Quantum Circuits

In the present noisy intermediate scale quantum computing era, there is a critical need to devise methods for the efficient implementation of gate-based variational quantum circuits. This ensures that a range of proposed applications can be deployed on real quantum hardware. The efficiency of quantum circuit is desired both in the number of trainable gates and the depth of the overall circuit. The major concern of barren plateaus has made this need for efficiency even more acute. The problem of efficient quantum circuit realization has been extensively studied in the literature to reduce gate complexity and circuit depth. Another important approach is to design a method to reduce the \emph{parameter complexity} in a variational quantum circuit. Existing methods include hyperparameter-based parameter pruning which introduces an additional challenge of finding the best hyperparameters for different applications. In this paper, we present \emph{QAdaPrune} - an adaptive parameter pruning algorithm that automatically determines the threshold and then intelligently prunes the redundant and non-performing parameters. We show that the resulting sparse parameter sets yield quantum circuits that perform comparably to the unpruned quantum circuits and in some cases may enhance trainability of the circuits even if the original quantum circuit gets stuck in a barren plateau.\\ \noindent{\bf Reproducibility}: The source code and data are available at \url{https://github.com/aicaffeinelife/QAdaPrune.git}

==> sections/abstract_iaai.tex <==
\begin{abstract}
In the current paradigm of quantum computing, parameterized quantum circuits are used to solve optimization problems using classical optimization algorithms running on a conventional computer. Scaling quantum computers to demonstrate ``quantum advantage" often requires solving large instance of optimization problems which in turn leads to deeper quantum circuits. However, the current generation of quantum devices struggle to reliably yield gradients for large depth circuits and hence struggle to obtain good solutions to the input problems. In this work, we explore emerging AI techniques to adaptively prune low impact parameters from a quantum circuit in order to help it scale effectively to larger problem instances. Our proposed procedure - QAdaPrune is a co-routine that can be run during the training of a quantum circuit to discover low impact parameters that can be pruned during the deployment phase. Experiments on different problems of interest in the quantum computing domain demonstrate that our process helps  scaling current quantum circuits to large instances of those problems which is essential in deploying quantum AI and other systems.\\
Reproducibility: Our code and results are available at \url{https://github.com/aicaffeinelife/QAdaPrune}.
\end{abstract}



==> sections/experiments.tex <==
\section{Experiments}\label{sec:expts}

In this section we shall demonstrate the effectiveness of our method on variety of VQA applications. In general, we will show that our method is able to identify and prune redundant parameters and cause minimal change in the final cost minima or accuracy on the given cost function and task. The source code and results are available at \url{https://github.com/aicaffeinelife/QAdaPrune.git}.

\subsection{Pruning and Trainability of VQCs}
In the first series of experiments, we aimed to establish if pruning parameters can help in training deeper or more complex circuits. In order to accomplish this, we instantiated a hardware efficient ansatz with alternating single qubit gates $R_X$ and $R_Y$. All qubits were then entangled in chained manner using Control-Z ($CZ$) gates. The numbers of layers was kept constant to $2$ and the number of qubits was varied from 2 to 8. We initialized the parameters from a uniform distribution $\bm{\theta} \sim Unif(-\pi, \pi)$ and optimized the circuit such that $U(\bm{\theta})\ket{0} = \ket{0}$, i.e., the VQC was supposed to learn the identity function. All circuits were optimized using a gradient descent optimizer with learning rate $0.2$. The results were obtained in the eigenbasis of the Pauli-Z global observable. A pruning window $w = 5$ was selected for all experiments.

The purpose of instantiating this circuit was that it is known to get stuck in barren plateaus as the number of qubits becomes higher when the parameters are initialized using the uniform distribution~\cite{cerezo2020cost}. Our hypothesis was that pruning can help in alleviating this phenomenon to some extent. Figure~\ref{fig:pruning_viability_study} shows the results of our experiments. We can observe that when no parameter pruning is employed, the circuit gets stuck in barren plateaus for $n > 6$ where $n$ is the number of qubits in circuit. However, when parameter pruning is employed, circuit gets into a barren plateau only after $n > 8$ and when the barren plateau does occur, the pruning algorithm automatically prunes all elements bringing the cost to zero. We can observe the resulting parameter sparsity in Figure~\ref{sfig:pruning_ratios}. Here, when the circuit is trainable, no parameter is pruned. When circuit starts to get stuck in barren plateaus, we are able to accomplish training by pruning $15 - 30\%$ parameters. These results show that an adaptive procedure like ours can help enhance trainability of VQCs. 
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/qnn_ansatz_fig.pdf}
    \caption{The ansatz used in QNN data classification experiments.}
    \label{fig:qnn_ansatz}
\end{figure}

\subsection{Quantum Data Classification With Pruning}

\begin{figure*}[t!]
\centering
\begin{subfigure}[t]{.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/iris_qnn_final_cost_comp.pdf}
    \caption{Cost Evolution}
    \label{sfig:qnn_fcost_comp}
\end{subfigure}
\begin{subfigure}[t]{.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/iris_qnn_final_acc.pdf}
    \caption{Final Accuracy Comparison}
    \label{sfig:qnn_facc_comp}
\end{subfigure}
\begin{subfigure}[t]{.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/qnn_iris_pruning_ratio_1.pdf}
    \caption{Pruning Ratios}
    \label{sfig:qnn_pruning_ratios}
\end{subfigure}

\caption{Results of running the QAdaPrune algorithm on different layer QNNs with Iris Dataset. Figures~\ref{sfig:qnn_fcost_comp} and~\ref{sfig:qnn_facc_comp} show the final cost and accuracy achieved by pruned and unpruned QNNs respectively. Figure~\ref{sfig:qnn_pruning_ratios} shows the percentage of parameters that were pruned by the QAdaPrune algorithm for different layers in the QNN.}
\label{fig:qnn_study}
\end{figure*}
% \is{I don't' understand the notation, should it be $x_i^j$?}
In the next series of experiments we consider the task of binary classification on a modified version of the Iris dataset~\cite{dua2019}  $\mathcal{D} = \{\bm{x}_i, y_i\}_{i=1}^{100}$ where $\bm{x}_i \in \mathbb{R}^{4}$ is the data and labels are  $y_i \in \{+1, -1\}$. To encode the classical data into a quantum state we employ angle embedding where for every $j^{th}$ component of data vector i.e. $x_i^j \in \bm{x}_i$ we prepare a rotation X gate with $x_i^j$ being the fixed angle rotation. Thus, for a single qubit $K(x_i^j) = R_X(x_i^j) = e^{-i\frac{x^j\sigma_x}{2}}$, where $\sigma_x$ is the Pauli-X matrix and is the gate generating Hermitian for the rotation X gate. We define our cost function 
\[
C(\bm{\theta}) = \frac{1}{M}\sum_{i=1}^{M} ||f(\ket{\psi(\bm{x}_i, \bm{\theta})}, \hat{\bm{O}})  - y_i||_2
\]
as the L2 distance between the expectation of the resulting quantum state $\ket{\psi(\bm{x}_i, \bm{\theta})}$ and the label $y_i$. In our experiment, $M = 100$. The ansatz used in our experiments is shown in Figure~\ref{fig:qnn_ansatz}.

In our experiments, we keep the number of qubits $n = 4$ due to the dimensionality of the input data points. We vary the layers from $4 \rightarrow 8$ and observe the performance of our algorithm. As before, we initialize our parameters from a uniform distribution over the interval $[-\pi, \pi]$. We use the RMSProp optimizer~\cite{tieleman2012lecture} with a step size of $0.1$. Each experiment is run for a 100 optimization steps with a pruning window $w = 5$ on a quantum device with $1000$ shots. The results of our experiments are shown in Figure~\ref{fig:qnn_study}.  From Figure~\ref{sfig:qnn_facc_comp} we can see that the pruned and unpruned QNNs achieve the same accuracy on the test set despite the pruned QNNs converging to slightly worse final minima (shown in Figure~\ref{sfig:qnn_fcost_comp}). Figure~\ref{sfig:qnn_pruning_ratios} shows the overall sparsity in the parameters after training. We can see for small depth circuits nearly $50\%$ parameters are pruned. For deeper circuits, our algorithm is still able to prune roughly $25\%$ of the parameters. This implies that with a dynamic pruning algorithm like ours, we can scale the training of QNNs to a larger depth without the concern of barren plateaus since the \emph{effective depth} of the circuit will be shallow. The effect of dynamic thresholding becomes more apparent when we consider the optimization trajectories of pruned and unpruned QNNs as shown in Figure~\ref{fig:qnn_opt_traj}. We can see that the height of spikes after each pruning step gets progressively lower and the network converges to similar minima as that of an unpruned QNN. The progressive lowering of the spikes can be attributed to the dynamic threshold adjustment that is central to our algorithm.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/iris_qnn_opt_traj.pdf}
    \caption{Optimization trajectory for pruned and unpruned four layer QNN on Iris
    dataset. Despite pruning a significant amount of parameters, a pruned QNN achieves similar minima as that of unpruned. The progressive lowering in spikes after each pruning window is due to adaptive threshold adjustment.}
    \label{fig:qnn_opt_traj}
\end{figure}


\subsection{Experiments with VQE}
We now focus our attention on the problem of estimating the ground state energy of a molecule using a VQC~\cite{VQE}. In our experiment, we consider estimating the ground state energy of a Hydrogen($H_2$) molecule with a UCCSD ansatz. We initialized the parameters from a normal distribution $\mathcal{N}(0, \pi)$ and used a gradient descent optimizer to run the algorithm for $40$ steps with a step size of $0.5$. The goal of our experiment was to investigate if our pruning algorithm can find redundant parameters in low parameter case. Figure~\ref{fig:vqe_cev} shows the energy estimation diagrams for the pruned and unpruned ansatz with the resulting parameter sparsity. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/vqe_uccsd_param_pruning.pdf}
    \caption{Energy estimation of $H_2$ molecule with and without pruning. After the last pruning step we are able to prune
    atleast $33\%$ parameters. }
    \label{fig:vqe_cev}
\end{figure}

We can observe that at step number 5, the trajectory changes with a slight increase in the energy estimate. This occurs when the algorithm discovers a redundant parameter and is pruned. However, the pruned ansatz is still able to achieve the energy estimate found by the unpruned ansatz. This demonstrates additional evidence to our claim that QAdaPrune is an effective pruning strategy that is automatically able to recognize and prune parameters with no significant impact on the performance of the VQC. 






==> sections/iaai_required_discussion.tex <==


\section{Deployment Challenges and Lessons Learned}

Our proposed algorithm is specifically developed for variational quantum circuits. In this section we discuss some relevant issues and lessons learned in deploying our algorithm to quantum circuits running on actual quantum hardware:\\ 

\noindent
\textbf{Costly Gradient Computation}: In the current setup of variational quantum computing, gradients of the cost function w.r.t. parameters are computed on the quantum device. This operation is not very computationally efficient since the only methods available for gradient computation are finite differences and parameter-shift-rule~\cite{schuld2019evaluating}. In both these methods, gradient computation requires at least two evaluations of the circuit leading to a quadratic cost of gradient computation. Our algorithm relies on gradient information to make decisions regarding pruning. The deployment challenge is to reduce the number of gradient computations required for making pruning decisions \cite{kulshrestha2023learning}.\\ 

\noindent
\textbf{Barren Plateaus}: As mentioned in previous sections, quantum circuits suffer from a barren plateau problem~\cite{mcclean2018barren} which cannot be easily remedied by techniques like residual connections. Due to this issue, the depth of quantum circuits is quite limited and they are unable to scale to large datasets. Our experiments on image classification datasets showed us that quantum circuits are unable to process $28 \times 28$ size images since the gradients get very small and our the pruning indices encompass the whole parameter set. We hope that advances in the quantum computing regime can help our algorithm to scale to these image sizes.\\


\noindent
\textbf{Hyperparameter Tuning}: Most pruning algorithms rely on hyperparameter driven heuristics to prune/regrow parameters~\cite{sim2021adaptive}. Our algorithm aims to keep these hyperparameters to minimum and make pruning decisions in a much more intelligent way. Nevertheless, we note that the optimal window size $w$ in our algorithm may require to be tuned to the dataset on which the quantum circuit is to be trained.\\ 


\noindent
\textbf{Scaling to Large Datasets}: In the current paper, we tried a QNN that consisted of small number of parameters. In order to establish QNNs as a viable alternative we need to scale the number of parameters and allow for processing large datasets. We interpret ``largeness" of the dataset in two ways. First, the size of the input is larger than MNIST or MNIST-like datasets and second the number of samples are greater than $1000$. In classical learning, scaling a DNN to handle such datasets often requires increasing the number of parameters. Scaling a QNN with large number of parameters is not straightforward due to the barren plateau issue mentioned above. The deployment challenge is to then apply our pruning algorithm to allow stable training of QNNs with large number of parameters.


 
% Expand the following points:
% 1. Creating deep random quantum circuits is hard
% 2. Deploying algorithm to actual quantum computer is quite involved process
% Open problems:
% 1. Scaling the algorithm to large amount of parameters
% 2. Deploying algorithm as a preprocessing step to a quantum transpiler



==> sections/introduction.tex <==
\section{Introduction}\label{sec:intro}
\begin{figure*}
\centering
\includegraphics[width=2\columnwidth]{figures/QAdaPrune.pdf}

\caption{Overall algorithmic flow of the QAdaPrune algorithm. Two key components of gradient importance and adaptive threshold are performed continuously until $t = nw$. When $ t\bmod w = 0$, a pruning index is built and the ineffective parameter components are pruned.}
\label{fig:qadaprune}
\end{figure*}
Quantum computing (QC) is an emerging technology that aims to revolutionize the general approach to computing~\cite{shor1994algorithms, collins1998deutsch}.  %While the realization of a fault-tolerant, scalable, and practical quantum computer is still a few years away, we can currently catch a glimpse of the possibilities offered by quantum computing in the Noisy Intermediate Scale Quantum (NISQ) regime. 
While the development of a fault-tolerant, scalable, and practical quantum computer remains a great challenge, and it is projected that significant advancements in this field will require a number of years to come to fruition, we can currently catch a glimpse of the possibilities offered by quantum computing in the Noisy Intermediate Scale Quantum (NISQ) regime. 
In this regime, we can experiment with the noisy quantum computers and obtain theoretical guarantees and insights on various aspects of quantum computers that will hold when fault-tolerant and scalable quantum architectures will be  realized.

Despite being far from perfect, NISQ-era quantum computers have become useful in exploring quantum advantages in a variety of domains due to the emergence of Variational Quantum Algorithms (VQAs)~\cite{cerezo2021variational}. Some of the examples include approximating solutions to such NP-hard problems as graph maxcut~\cite{farhi2014qaoa_for_bounded, qaoa20142}, minimum graph partitioning \cite{ushijima2021multilevel}, community detection \cite{shaydulin2019network,liu2022layer}, estimating the ground state energy of molecules~\cite{VQE}, portfolio optimization \cite{herman2022survey}, pattern recognition~\cite{farhi2018classification}, unsupervised data compression~\cite{romero2017quantum} and even circuit architecture search~\cite{du2022quantum}. 

The current paradigm of VQAs envisions a hybrid approach where a Variational Quantum Circuit (VQC) is deployed on a quantum device with gates parameterized by real valued parameters. The parameters are optimized using a classical optimization algorithm (e.g., gradient descent) running on a classical computer. The VQC input is a vector of parameters and the output is the gradient estimate and the current cost function estimate. The overall goal is to obtain a set of parameters that corresponds to some optimal point of the cost function (e.g., global 
 maximum or minimum). 

%% potentially add a table summarizing current methods on efficient 
%% gate design. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=.5\columnwidth]{figures/qadaprune_v1.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

Theoretically, the VQC may be able to approximate an arbitrary function $f: \mathbb{C} \mapsto \mathbb{R}$  if infinite resources are available for simulation on a quantum device. However, in practice, the limited gate depth of current generation quantum computers and the inherent sensitivity of qubits to noise make it extremely hard to approximate such functions efficiently. This limitation has led to development of methods to produce low-resource circuits that can learn an optimal function $f^*$ from a given family of all possible functions in Hilbert space (collectively called as the set of hypothesis functions $\mathcal{H}$)~\cite{arunachalam2020quantum}. These methods fall in two broad categories. The first category consists of circuit level methods that include transpiling of a complex simulator circuit into an efficient gate level physical circuit~\cite{rakyta2022efficient}, generating efficient quantum circuits from a known ``supercircuit"~\cite{du2022quantum}. The second category consists of methods that aim to reduce circuit complexity by employing some version of parameter pruning. For instance, Wang~\emph{et al.}~\cite{wang2022qoc} propose utilizing parameter shift rules~\cite{schuld2019evaluating} to evaluate gradient on chip and a probabilisitc gradient pruning algorithm to remove ineffective parameters. Hu~\emph{et al.}~\cite{hu2022quantum} propose a compression pipleine which involves alternate pruning and quantization steps to reduce the overall number of parameters in the circuit. Yet another method is introduced by Sukin~\emph{et al.}~\cite{sim2021adaptive} where an online parameter pruning method is proposed. It adaptively prunes and grows parameters based on four input hyperparameters - the global sparsity, number of parameters to prune at a given timestep, pruning threshold and tolerance value.  


\emph{Our contributions:} To the best of our knowledge, no pruning algorithm considers having independent thresholds for different parameter components. Instead, the decision to prune a particular parameter component is guided by comparing that component's performance against some scalar threshold which is either accepted as input or adjusted in an online fashion during training. A critical examination of existing works in this direction raises two key concerns about the pruning framework:
\begin{itemize}
    \item Can a global threshold effectively determine the relevance of each parameter component?
    \item Is there a more nuanced and effective criteria than gradient magnitude for pruning? 
\end{itemize}

% \is{What is missing here is a a few sentences in the spirit ``without addressing these concerns properly, the quantum circuits may suffer ...}
In contrast to neural networks where neurons often encode redundant information, the parameters of variational circuits evolve more freely due to limited entanglements in the circuits. Thus, a single scalar threshold may not be able to capture the true importance of a parameter component and may even lead to a degradation of performance by incorrectly deleting essential parameters.  

In this paper, we address these questions by introducing the \textbf{\emph{QAdaPrune}} algorithm, which independently adapts the threshold of each parameter component and uses information from the optimization trajectory to make pruning decisions. We empirically show that our algorithm is able to determine redundant parameters with very little effect on the final extrema and other metric values associated with the computation. We further demonstrate that by pruning irrelevant parameters our algorithm is able to enhance trainability of quantum circuits which may otherwise get stuck in a barren plateau. 

% Parameter based pruning methods make implicit assumptions in the way the parameters are classified as ``irrelevant" to the given cost function. In general, these methods utilize a global threshold to determine parameter relevance. It is generally assumed that the global threshold is an input to the algorithm or a hyperparameter that needs to be tuned over several runs of the pruning procedure. The existing body of work leaves two key questions unanswered in parameter pruning: First, can the parameter relevance be solely determined by a global threshold? Second, is comparing magnitude of gradient of the cost function w.r.t parameter enough to determine if the parameter must be pruned?. 

% In this paper, we address these questions by proposing the \textbf{\emph{QAdaPrune}} algorithm which adaptively determines the \emph{component wise} parameter thresholds and utilizes a novel criteria for pruning parameters. We show that our algorithm is able to enhance the trainability of circuits which are known to get stuck in barren plateaus and demonstrate that our algorithm is able to prune a significant amount of parameters while still yielding similar cost function minima and accuracy. Based on our experiments we then advance the \emph{redundant representation hypothesis} which we believe may lead to significantly better VQC designs in the future. 



